TraceMesh: Scalable and Streaming Sampling for Distributed Traces

Distributed tracing serves as a fundamental element in the monitoring of cloud-based and datacenter systems. It provides visibility into the full lifecycle of a request or operation across multiple services, which is essential for understanding system dependencies and performance bottlenecks. To mitigate computational and storage overheads, most tracing frameworks adopt a uniform sampling strategy, which inevitably captures overlapping and redundant information. More advanced methods employ learning-based approaches to bias the sampling toward more informative traces. However, existing methods fall short of considering the high-dimensional and dynamic nature of trace data, which is essential for the production deployment of trace sampling. To address these practical challenges, in this paper we present TraceMesh, a scalable and streaming sampler for distributed traces. TraceMesh employs Locality-Sensitivity Hashing (LSH) to improve sampling efficiency by projecting traces into a low-dimensional space while preserving their similarity. In this process, TraceMesh accommodates previously unseen trace features in a unified and streamlined way. Subsequently, TraceMesh samples traces through evolving clustering, which dynamically adjusts the sampling decision to avoid over-sampling of recurring traces. The proposed method is evaluated with trace data collected from both open-source microservice benchmarks and production service systems. Experimental results demonstrate that TraceMesh outperforms state-of-the-art methods by a significant margin in both sampling accuracy and efficiency.

==> sections/06-related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Distributed tracing has emerged as a crucial tool for understanding and optimizing complex service-oriented architectures.
It provides an invaluable mechanism for tracking requests as they navigate through the intertwined services of a distributed system, enabling developers to identify bottlenecks, spot inefficiencies, and troubleshoot performance issues.
This area of study has seen significant contributions from various efforts.
X-Trace~\cite{DBLP:conf/nsdi/FonsecaPKSS07} aims to provide a comprehensive view of service behavior across multiple system layers.
Dapper~\cite{sigelman2010dapper} is a distributed system tracing infrastructure developed by Google.
Its design goals include low overhead, application-level transparency, and ubiquitous deployment across extensive, large-scale systems.
Pivot Tracing~\cite{DBLP:conf/sosp/MaceRF15} considers the \textit{happened-before} relations between events during dynamic instrumentation.
This provides users with the ability to define arbitrary metrics for mining useful information about root causes at runtime.
Canopy~\cite{DBLP:conf/sosp/KaldorMBGKOOSSV17}, developed by Facebook, is an end-to-end performance tracing infrastructure.
It captures performance data with causal relationships across various platforms including browsers, mobile applications, and backend services.
This aids engineers in querying and analyzing performance data in real-time.
DeepFlow~\cite{DBLP:conf/sigcomm/ShenZXSLSZWY0XL23} is a non-intrusive distributed tracing framework for troubleshooting microservices.
It provides out-of-the-box tracing via a network-centric tracing plane and implicit context propagation.
In recent years, open-source tracing frameworks like Jaeger~\cite{jaeger} and Zipkin~\cite{zipkin} have seen widespread adoption in practical applications.

Besides the infrastructure for generating distributed traces, trace data are widely used in various system reliability assurance tasks.
The empirical study in~\cite{DBLP:journals/tse/ZhouPXSJLD21} shows that the current industrial practices of microservice debugging can be improved through the application of appropriate tracing and visualization techniques.
MEPFL~\cite{DBLP:conf/sigsoft/Zhou0X0JLXH19} leverages system trace logs in the production environment to predict latent errors, faulty microservices, and fault types at runtime.
Groot~\cite{DBLP:conf/kbse/WangWJHWKX21} builds a real-time causality graph to facilitate root cause analysis in microservices, which allows adaptive customization of link construction rules to incorporate domain knowledge.
TraceStream~\cite{DBLP:conf/issre/ZhouZPYLLZZD23} identifies potential clusters of anomalous traces within evolving trace data and employs spectral analysis to pinpoint the specific 
anomalous services.
Some work~\cite{DBLP:conf/kbse/ChenLSZWLYL21,DBLP:conf/icse/LeeYCSL23,DBLP:conf/sigsoft/YuCLCLZ23} utilizes a multi-modal approach, which integrates traces with logs and metrics to provide more comprehensive information about system status for microservice troubleshooting.
Traces also serve a crucial role in in analyzing system dependencies~\cite{DBLP:conf/cloud/LuoXLYXZDH021}, critical paths~\cite{DBLP:conf/usenix/0002RRPSC22}, resource characterization~\cite{DBLP:conf/icpp/WangLWJCWDXHYZ22,DBLP:conf/kbse/LiuJGHCFYYL23}, and microservice architecture~\cite{DBLP:conf/usenix/HuyeSS23,DBLP:conf/sigsoft/0001ZZIGC22}.
This enables developers to identify bottlenecks, spot inefficiencies, and subsequently optimize the overall system performance.

With the dramatic increase in trace volume in production systems, trace sampling has become an essential technique to manage data overload and maintain system efficiency.
Representative approaches are introduced in Section~\ref{sec:baselines}, which leverage a variety of methods, including tree-based models~\cite{DBLP:conf/icws/HuangCYCZ21,DBLP:conf/noms/GiasGSPOC23}, clustering algorithms~\cite{DBLP:conf/cloud/Las-CasasMGF18}, and neural language techniques~\cite{DBLP:conf/cloud/Las-CasasPAM19}.
STEAM~\cite{DBLP:conf/sigsoft/HeFLZ0LR023} preserves system observability by sampling mutually dissimilar traces.
It employs Graph Neural Networks (GNN) for trace representation~\cite{DBLP:conf/sigsoft/Zhang0ZSYCY22}, and requires human labeling to incorporate domain knowledge.
Hindsight~\cite{DBLP:conf/nsdi/ZhangXAVM23} introduces the idea of \textit{retroactive sampling}.
Instead of eagerly ingesting and processing traces, it lazily retrieves trace data only after symptoms of a problem are detected.
Hindsight is based on the observation that the generation of traces at nodes is not expensive, but the ingestion of trace data is resource-intensive.
Thus, tail sampling strategy can be applied to achieve accurate trace sampling without occurring too much runtime overhead (\ie before the processing of trace data).

While progress has been made, existing learning-based approaches for trace sampling lack consideration of practical challenges associated with their deployment in production environments.
Specifically, the large volume of trace data and feature space demand a highly efficient solution.
The diversity of traces also requires fast ability to accommodate new dimensions.
Unlike these works, our design emphasizes operational efficiency and flexibility.
It not only handles large volumes of trace data with a vast feature space, but also quickly adapts to the emergence of unprecedented trace features.

==> sections/07-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we propose \name, a scalable and streaming trace sampler.
It addresses the practical challenges of deploying trace sampling techniques in production systems, which have not been adequately addressed in existing work.
The scale and complexity of modern service systems render trace data highly diverse and dynamic.
The unpredictable system updates and user behaviors further compound the situation.
Thus, a practical sampler should be able to handle the vast feature space of traces and quickly generalize to previously unknown features within the trace stream.
To this end, we first perform trace vector encoding by considering both the structural and temporal features.
Next, we employ streaming Locality-Sensitivity Hashing (LSH) technique to enable efficient trace similarity mining by projecting them into a low-dimensional space.
In this process, new features can be seamlessly incorporated without changing the input dimensionality.
Finally, given a sampling budget, we identify and capture uncommon traces through evolving clustering.
We dynamically adjust the sampling decision to prevent accumulating redundant information.
We have evaluated \name using trace data collected from both open-source microservice benchmarks and production service systems.
Experimental results highlight its potential to pave the way for efficient system monitoring.

==> sections/08-acks.tex <==
% \vspace{-2pt}
\section*{Acknowledgement}

This work is supported by the National Natural Science Foundation of China (No. 62202511) and the Research Grants Council of the Hong Kong Special Administrative Region, China (No. CUHK 14206921 of the General Research Fund).

% The work was supported by Key-Area Research and Development Program of Guangdong Province (No. 2020B010165002), the Research Grants Council of the Hong Kong SAR, China (CUHK 14206921), and Australian Research Council (ARC) Discovery Project (DP200102940).
